Under-the-barrier electron-ion interaction during tunnel ionization

We consider tunnel ionization of an atom or molecule in a strong field within an analytical treatment of the R-matrix method, in which an imaginary boundary is set up inside the classically forbidden region that acts as a source of ionized electrons. These electrons are then propagated in the semiclassical approximation, and relying on a numerical solution of the inner region, which is accessible using quantum chemical techniques, we describe the subsequent evolution of the ionized electron and the ionic core. Importantly, we show that correlation interactions between the ionized electrons and those left behind in the core can play a role during ionization, and that interactions can occur while the electron is still inside the classically forbidden region that enable tunnelling from channels normally subject to far greater exponential suppression since they are subject to higher and wider tunnelling barriers. This interaction can be described analytically using saddle-point methods that find the dominant contributions to the temporal, spatial and momentum integrals that make up the expressions for the ionization yield. However, these methods yield results for the angular distributions of the ionized electron that do not necessarily match experiment and which yield physically unsatisfactory solutions. In this report we develop a formalism to evaluate these integrals exactly, which yields more precise calculations of the angular distributions while at the same time providing the language, in terms of exchange of angular momentum, with which to understand their origins and their differences from previous cases, thus giving an insight into the fundamental physics of the correlation interaction process.

==> conclusions.tex <==


%\chapter{Conclusions}
some brief conclusions
























==> currentwork.tex <==


\chapter{Current work}

Misha:

At the moment I know how the last integral, over $t''$, looks, but I'm a bit uncertain as to how to go about it. Ignoring the detail of the numerical coefficients, it looks like


\begin{align*}
	a_m^{(2)}(\vbp)
	& = 
	(\textrm{coefficients})\times 
	a_g(t_s)
	e^{iI_{p,n}t_s}
	\times(\textrm{phases}) \times
	e^{iW_C}
	\frac{K_0}{\sqrt{S_V''}}
	\\ & \qquad \times
	e^{i(m+\mu)\phi_p} p_\perp^{|m+\mu|}
	e^{-\frac{i}{2}\int_{t_s}^T (\vbp+\vb{A}(\tau))^2\d\tau}
	\sum_j  (\textrm{coefs})
	\times \\ & \qquad
	\int_0^{\tauT}\d\xi
	\frac{
	   b_m(t_0,t'') b_n(t'',ts) Q_{\lambda\mu} (t'')
	   }{
	   \left(\int_{t_s}^{t''}(p_\parallel+A(\tau))\d\tau\right)^{\lambda+\mu+2j+1}
	}
	L_{\frac{|m|+|\mu|-|m+\mu|}{2}+j}^{(|m+\mu|)}(\frac{1}{2}\xi p_\perp^2)
	\xi^{\frac{|m+\mu|+|\mu|-|m|}{2}+j}
	e^{-\Delta I_p \xi}.
\end{align*}
Here of course $t''=t_0+i\xi$, the $b_n$ are Stark shifts, $Q_{\lambda\mu}$ is the multipole moment, which depends on the matrix element $\matrixel{m(t'')}{V(t'')}{n(t'')}$, and the integral in the denominator is the factor $1/z^\textrm{power}$. The power of $\xi$ and the degree of the polynomial are always positive and any combination of positive power and degree is reachable with suitable $m$ and $\mu$ (though these may be relatively large).

I'm leaning towards seeing the integral as something like
$$
	\int_0^{\tauT}\d\xi
	(\textrm{slow factors})\times
	\xi^{\frac{|m+\mu|+|\mu|-|m|}{2}+j}
	e^{-\Delta I_p \xi}
$$
and then evaluating the slow terms at the maximum of the factor $\xi^\textrm{power}	e^{-\Delta I_p \xi}$. The main and crucial difference, as I see it, is that the presence of the power of $\xi$ pushes the main contribution to the integral away from $\xi=0$ so that the correlation interaction primarily occurs at some definite time \textit{before} the tunnel exit.

Another thing to consider is how the three energy scales present, $\Delta I_p$, $p_\perp^2$ and $\frac{1}{\tauT}$, play off each other, since depending on their relative sizes, for example, the oscillations in the Laguerre polynomial may become invisible or may severely reduce the integral, or even introduce multiple maxima at which to evaluate the other slow factors. (In particular, I'm thinking of the case where $p_\perp^2\approx \Delta I_p$ and $\Delta I_p\tau\gg 1$, where ignoring the slow factors the integral $\int L_1(\xi)e^{-\xi}\d\xi$ is zero or close to that.) Just another thing to think about.















